Pair DETR: Contrastive Learning Speeds Up DETR Training

The DETR object detection approach applies the transformer encoder and decoder architecture to detect objects and achieves promising performance. In this paper, we present a simple approach to address the main problem of DETR, the slow convergence, by using representation learning technique. In this approach, we detect an object bounding box as a pair of keypoints, the top-left corner and the center, using two decoders. By detecting objects as paired keypoints, the model builds up a joint classification and pair association on the output queries from two decoders. For the pair association we propose utilizing contrastive self-supervised learning algorithm without requiring specialized architecture. Experimental results on MS COCO dataset show that Pair DETR can converge at least 10x faster than original DETR and 1.5x faster than Conditional DETR during training, while having consistently higher Average Precision scores.

==> Pair DETR-2/fig/overview.tex <==
%\begin{figure*}
%\begin{center}
%\includegraphics[width=.8\columnwidth]{fig/Fig2_overall.png}
%\hfill
%\includegraphics[width=.99\columnwidth]{fig/Contrastive.png}
%\end{center}
%\caption{
% 
%\textbf{Outline -- }
%A figure summarizing the entire algorithm
%}
%\label{fig:overview}
%\end{figure*}

%\begin{figure*}[t!]
%    \centering
%    \begin{subfigure}[t]{0.5\textwidth}
%        \centering
%        \includegraphics[height=2.7in]{fig/Fig2_overall.png}
%        \caption{Overall Framework in training}
%    \end{subfigure}%
%    ~ 
%    \begin{subfigure}[t]{0.5\textwidth}
%        \centering
%        \includegraphics[height=2in]{fig/Contrastive.png}
%        \caption{Detail of contrastive learning}
%    \end{subfigure}
%    \caption{(a) Depicts the overall decoder architecture and training procedure of Pair-Detr. For the sake of brevity backbone network (CNN) and encoder and its output (keys for cross-attention in decoders) are not shown. (b) Detail of contrastive learning used in model. Pair-DETR jointly trains an Top-left and Center decoders and maximize the similarity between top-left and center pairs.}
%\end{figure*}


\begin{figure*}
\centering
\includegraphics[width=0.6\textwidth]{fig/Overall_final.png}
\caption{\textbf{Pair DETR} contains additional decoder comparing to the other DETR based detection models. One decoder is dedicated to detection of center points (Center decoder) and the other is dedicated to locating top-left points (Top-left decoder). Pair DETR is optimized jointly using classification and regression losses for each decoder and contrastive loss between the two mentioned decoders.  }
\label{fig:method_overall}
\end{figure*}

==> Pair DETR-2/fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> Pair DETR-2/sec/0_abstract.tex <==
\begin{abstract}
The DETR object detection approach applies the transformer encoder and decoder architecture to detect objects and achieves promising performance. In this paper, we present a simple approach to address the main problem of DETR, the slow convergence, by using representation learning technique. In this approach, we detect an object bounding box as a pair of keypoints, the top-left corner and the center, using two decoders. By detecting objects as paired keypoints, the model builds up a joint classification and pair association on the output queries from two decoders. For the pair association we propose utilizing contrastive self-supervised learning algorithm without requiring specialized architecture. Experimental results on MS COCO dataset show that Pair DETR can converge at least 10x faster than original DETR and 1.5x faster than Conditional DETR during training, while having consistently higher Average Precision scores.
%achieves 42.2\% AP using R-50 backbone on MS COCO dataset, outperforming DETR and Conditional DETR.  
\end{abstract}

==> Pair DETR-2/sec/0_metadata.tex <==
\title{Pair DETR: Contrastive Learning Speeds Up DETR Training}

\author{Seyed Mehdi Iranmanesh\\
Amazon \\
{\tt\small mehdiir@amazon.com}
 %For a paper whose authors are all at the same institution,
 %omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
 \and
 Xiaotong Chen\\
 University of California, Santa Barbara\\
 {\tt\small xchen774@umail.ucsb.edu}
  \and
 Kuo-Chin Lien\\
 Appen\\
 {\tt\small klien@appen.com}
}

==> Pair DETR-2/sec/1_introduction.tex <==
\section{Introduction}
 Object detection utilizing transformers (DETR)~\cite{carion2020end} is a recent approach that represents object detection as a direct prediction problem via a transformer encoder-decoder~\cite{vaswani2017attention}. DETR reaches a competitive performance with Faster R-CNN~\cite{ren2015faster} without using hand-designed sample selection and non-maximum suppression (NMS). However, DETR approach suffers from slow convergence on training, which needs large-scale training data and long training epochs to get good performance.
 
\begin{figure}
\centering
\begin{tabular}{cc} 
\includegraphics[height=0.7\columnwidth,keepaspectratio]{fig/Firstfigb1.png} \\ (a) \\ \includegraphics[height=0.7\columnwidth,keepaspectratio]{fig/Firstfiga.png} \\
(b)
\end{tabular}
\caption{Transformer based detection models such as DETR~\cite{carion2020end} and Deformable DETR~\cite{zhu2020deformable} rely only on detecting center points (\ref{fig:introduction}a). Pair DETR proposes to detect additional point namely Top-left to localize objects more effectively (\ref{fig:introduction}b).  }
\label{fig:introduction}
\end{figure}
 
\if 0
\begin{figure}
\begin{subfigure}[b]{\columnwidth}
\centering
\includegraphics[width=0.8\columnwidth]{fig/Firstfig_b (1).png}
\caption{Detection using DETR approach (Solely rely on center points).}
\label{fig:introduction_detr}
\end{subfigure}
\vspace{0.05cm}

\begin{subfigure}[b]{\columnwidth}
\centering
\includegraphics[width=0.8\columnwidth]{fig/First_fig_a.png}
\caption{Detection using proposed Pair DETR approach (Considers two important points).}
\label{fig:introduction_pairdetr}
\end{subfigure}
\vspace{0.05cm}

\caption{Transformer based detection models such as DETR~\cite{carion2020end} and Deformable DETR~\cite{zhu2020deformable} rely only on detecting center points (\ref{fig:introduction_detr}). Pair DETR proposes to detect additional point namely Top-left to localize objects more effectively (\ref{fig:introduction_pairdetr}).  }
\label{fig:introduction}
\end{figure}
\fi 
 
 
DETR~\cite{carion2020end} uses a set of learned object queries to reason about the associations of the objects and the global image context to output the final predictions set. However, the learned object query is very hard to explain. It does not have a distinct meaning and the corresponding prediction slots of each object query do not have a unique mode.

Deformable DETR~\cite{zhu2020deformable}, handles the issues of DETR by replacing the global dense attention (self-attention and cross-attention) with deformable attention that attends to a small set of key sampling points and using the high-resolution and multi-scale encoder. This however reduced their AP on the bigger objects which needs global dense attention.
 
Conditional DETR~\cite{meng2021conditional} approach is motivated by high dependence on content embeddings and minor contributions made by the spatial embeddings in cross-attention mechanism in DETR. The experimental results in DETR ~\cite{carion2020end} illustrate that if removing the positional embeddings in keys and the object queries from the decoder layer and only using the content embeddings in keys and queries, the detection AP drops. The AP reduction is more observable when the positional embeddings are dropped from the decoder compared the the case when they are dropped from the encoder. 

Conditional DETR approach, learns a conditional spatial embedding for each query from the corresponding previous decoder output embedding. It shrinks the spatial range for the content queries to localize the effective regions for class and box prediction. As a result, the dependence on the content embeddings is less and the training is easier.

 
Inspired by the great success of contrastive learning and self-supervised training in different applications such as CLIP~\cite{radford2021learning} and SimCLR~\cite{chen2020simple}, we aim to utilize it in transformer training of DETR.
 
Two corner points, e.g. the top-left and bottom-right corners, can define the spatial extent of a bounding box, providing an alternative to the typical 4-d descriptor consisting of the box’s center point and size which is also used in DETR. This has been used in several bottom-up object detection methods such as~\cite{law2018cornernet,zhou2019bottom,tychsen2017denet} and has shown significantly better performance in object localization but not object classification~\cite{chen2020reppoints}.
%, as seen in Table 1. In later sections, we show that this verification task can
%complement regression based methods to obtain more accurate object localization.

In order to take advantage of a better localization we propose Pair DETR which consists of a pair of decoders, namely Center decoder and Top-left decoder. Center decoder is responsible to detect the center of bounding boxes while top-left decoder task is to predict top-left of the corresponding bounding boxes (see Fig.\ref{fig:introduction}). In addition to the center prediction, the center decoder is responsible for class prediction and the top-left decoder obeys the classification decision. The learned object queries are shared between two decoders, and as a result the order of center and top-left outputs are the same. To have a more discriminative embedding, contrastive learning approach is utilize between these two sets of output. The contributions of the paper are summarized as follows:

\begin{itemize}
\item We propose to use contrastive learning on features of two decoders to improve the embedding subspace of decoder and improve the classification performance. 
\item We incorporate an extra keypoint \emph{Top-left} and associate it with the the standard keypoint -- center of a bounding box. This novel two-point Transformer architecture improves the localization performance. 
\item  Extensive experiments are conducted to prove the effectiveness of the proposed model comparing to state-of-the-art on COCO dataset. 
\end{itemize}
 


==> Pair DETR-2/sec/2_related.tex <==
\input{fig/overview} %< bloody latex and its heuristics for figure placement

\section{Related works}
\subsection{Convolution based object detection}

Most object detection models make predictions from carefully designed initial guesses. Anchor boxes or object centers are two main approaches for making the initial guesses. Anchor based solutions which borrow the idea from the proposal based models, can be categorized into two-stage models such as Faster RCNN~\cite{ren2015faster} variants, and one-stage approaches such as SSD~\cite{liu2016ssd}, and YOLO~\cite{redmon2016you}. 

Two-stage detectors generate a sparse set of regions of interest (RoIs) and classify each of them by a network. Faster RCNN~\cite{ren2015faster} introduced a region proposal network (RPN), which generates proposals from a set of pre-determined candidate boxes, namely anchor boxes. R-FCN~\cite{dai2016r} further improves the efficiency of Faster-RCNN by replacing the fully connected sub-detection network with a fully convolutional sub-detection network. DeNet~\cite{tychsen2017denet} is a two-stage detector which generates RoIs without using anchor boxes. It determines how likely each location belongs to either the  top-right, top-left, bottom-right, or bottom-left corner of a bounding box. It then creates RoIs by enumerating all possible corner combinations, and performs the standard two-stage approach to classify each RoI.


One-stage detectors such as SSD and YOLO, remove the RoI pooling step and detects objects in a single network. One-stage detectors are usually more computationally efficient than two-stage detectors while maintaining comparable performance on different challenging benchmarks. SSD  directly classifies and refines anchor boxes that are densely defined over feature maps at different scales. YOLOv1~\cite{redmon2016you} predicts bounding boxes directly from an image, and later is improved in YOLOv2~\cite{redmon2017yolo9000} by utilizing anchors.

Anchor-free models such as YOLOv1, instead of using anchor boxes, predict bounding boxes at points near the center of objects. Only the points near the center are used since they are considered to be able to produce higher quality detection. YOLOv1 struggles with low recall, and thus YOLOv2 chooses to go back employing anchor boxes. Compared to YOLOv1, FCOS~\cite{tian2019fcos} can utilize all points in a ground truth bounding box to predict the bounding boxes and make comparable results to anchor based solutions. CenterNet~\cite{zhou2019objects} predicts the center, width, and height of objects with hourglass networks, demonstrating promising performance. CornerNet~\cite{law2018cornernet} is another keypoint-based approach, which directly detects an object using a pair of corners and groups them to form the final bounding box. 

\subsection{Transformer based object detection}

DETR successfully applies Transformers to object detection, effectively removing the need for many hand-designed components like non-maximum suppression or anchor generation. The high computation complexity issue, caused by the global encoder self attention, is handled by sparse attentions in Deformable DETR~\cite{zhu2020deformable} or by utilizing adaptive clustering transformer~\cite{zheng2020end}. Deformable DETR~\cite{zhu2020deformable} is introduced to restrict each object query to attend to a small set of key sampling points around the reference points, instead of all points in feature map. Using multi-scaling and utilizing high resolution feature maps, it can mitigate potential losses in the detection of small objects.

The other critical issue, slow training convergence in DETR~\cite{carion2020end}, has been attracting a lot of recent research attention. Deformable DETR~\cite{zhu2020deformable} adopts deformable attention to replace decoder cross-attention. TSP approach~\cite{sun2021rethinking} combines the FCOS and R-CNN-like detection heads and removes the cross-attention modules. With unsupervised pre-training of the transformers, UP-DETR~\cite{dai2021up} enhances DETR performance on object detection precision and also speed of model convergence. Conditional DETR~\cite{meng2021conditional} encodes the reference point as the query position embedding. It utilizes the reference point to generate position embedding as the conditional spatial embedding in the cross-attention layers.  Using spatial queries shrinks the spatial range for the content queries to localize the regions for box and class prediction. Therefore, the dependence on the content embeddings is relaxed and the training convergence is faster. Our proposed approach is based on conditional DETR to improve the performance of DETR object detection while taking advantage of conditional DETR architecture for faster training convergence. 




==> Pair DETR-2/sec/3_method.tex <==
\section{Methodology}
In this section, we first introduce preliminaries and then discuss details of our method.
\subsection{Contrastive learning}
Contrastive learning has become popular due to
leading state-of-the-art results in different unsupervised representation learning tasks. The goal is to learn representations by contrasting positive pairs against negative pairs~\cite{hadsell2006dimensionality} and is used in various computer vision tasks, including data augmentation~\cite{oord2018representation}, or diverse scene generation~\cite{tian2020contrastive}. The main idea of contrastive learning is to move the similar pairs near and dissimilar pairs far in the embedding subspace.

\begin{figure*}
\centering
\includegraphics[width=0.6\textwidth]{fig/Contrastive.png}
\caption{Pair DETR utilizes contrastive learning to maximize the similarity between corresponding output embeddings (positive) of Center and Top-left decoders and minimizing the similarity to other output embeddings (negatives). }
\label{fig:contrastive}
\end{figure*}

In this work, we follow a similar approach to SimCLR framework~\cite{chen2020simple} for contrastive learning. SimCLR consists of four main components: a stochastic data augmentation method which generates positive pairs, an encoding network ($\mathrm{f}$) that extracts the embedding representation vectors from augmented samples, a small projector head ($\mathrm{g}$) that maps representations to the loss space, and a contrastive loss function that enforces more discriminative embedding representation between positive and negative pairs. Given a random mini-batch of N samples, SimCLR generates N positive pairs using the data
augmentation method. For all positive pairs, the remaining 2N-1 augmented samples are treated as negative examples. Let $\mathrm{h_i = f(x_i)}$ be the representations of all 2N
samples and $\mathrm{z_i = g(h_i)}$ be the projections of these representations. Let $\mathrm{sim(u, v) = u^Tv /||u|| ||v||}$ denote the dot product between $\ell_2$ normalized u and v. Then the loss function for a positive pair of examples (i, j) is defined as:
\begin{align}\label{eq1} 
	\ell_{i,j} = -\log \dfrac{\exp({\mathrm{sim(z_i,z_j)/\tau}})}{\Sigma^{2N}_{k=1}\mathbb{1}_{[k\neq {i}]}\exp({\mathrm{sim(z_i,z_j)/\tau}})}   ,
\end{align}
where $\mathbb{1} \in \{0, 1\}$ is an indicator function evaluating to
1 iff $\mathrm{\{k\neq {i}\}}$ and $\tau$ denotes a temperature parameter. The final loss which is also known as $\emph{NT-Xent}$~\cite {sohn2016improved,oord2018representation} considers the average of losses computed across all positive pairs, both (i, j) and (j, i), in a mini-batch~\cite{chen2020simple}.



\subsection{DETR}
The proposed approach follows detection transformer (DETR) and predicts all the objects at once without the need for anchor generation or NMS. DETR architecture consists of a CNN backbone, a transformer encoder, a transformer decoder, and object class and box position predictors. The goal of transformer encoder is to enhance the embeddings output from the CNN backbone. It is a stack of multiple encoder layers, where each layer mainly consists of a self-attention layer and a feed-forward layer. 

The transformer decoder is a stack of decoder layers. Each decoder layer, consists of three main components which are  self-attention, cross-attention, and feed-forward layers, respectively. Self-attention layer performs interactions between the embeddings, outputted from the previous decoder layer and is utilized to remove duplication in prediction. Cross-attention layer combines the embeddings output from the encoder to refine the decoder embeddings for enhancing class and box prediction. Conditional DETR utilizes conditional cross-attention mechanism and forms the query by concatenating the content query $\mathrm{c_q}$, outputting from decoder self-attention, and the spatial query $\mathrm{p_q}$.
\subsection{Pair DETR}

The proposed Pair DETR mechanism forms by creating a pair of points. There are evidences which show the superiority of using two corners (e.g. the top-left corner and
bottom-right corner) in terms of localization comparing to the other forms of object detection models which using center, width, height of bounding box representation. However, corner based models in general perform worse for the classification part [3]. One possible reason might be due to the fact that the corners contain less contextual information of the object inside the bounding box comparing to the center.
Pair DETR is to taking advantage of both of these models by considering a pair of the center of bounding box and one corner of the same bounding box. Having only one corner in addition to the center is enough since the bottom-right corner is reciprocal to the top-left one. In addition, to associate the corresponding points belonging to the same bounding box, the center and one corner probably have more similar contents comparing to two opposite corners.

\begin{table*}[]
\centering
\caption{Comparison between Pair DETR and previous DETR variants on COCO 2017 val. Our Pair DETR approach for all the backbones including high resolution (DC5-R50 and DC5-R101) and low resolution (R50 and R101) is at least 10× faster than the original DETR. In addition, Pair DETR performs almost 1.5$\times$ faster than conditional DETR. Pair DETR is empirically superior to other two single-scale DETR variants.}
\begin{tabular}{llllllll}
\hline
Model                            & \multicolumn{1}{l|}{\#epochs} & AP   & AP$_{50}$ & A$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_L$ \\ \hline
DETR-R50                         & \multicolumn{1}{c|}{500}      & 42.0 & 62.4      & 44.2     & 20.5   & 45.8    & 61.1    \\
DETR-R50                         & \multicolumn{1}{c|}{50}       & 34.9 & 55.5      & 36.0     & 14.4   & 37.2    & 54.5    \\
Conditional DETR-R50             & \multicolumn{1}{c|}{50}       & 40.9 & 61.8      & 43.3     & 20.8   & 44.6    & 59.2    \\
Conditional DETR-R50             & \multicolumn{1}{c|}{75}       & 42.1 & 62.9      & 44.8     & 21.6   & 45.4    & 60.2    \\
Conditional DETR-R50             & \multicolumn{1}{c|}{108}      & 43.0 & 64.0      & 45.7     & 22.7   & 46.7    & 61.5    \\
Pair DETR-R50                    & \multicolumn{1}{c|}{50}       & 42.2 & 63.4      & 44.9     & 21.5   & 45.5    & 61.1    \\
Pair DETR-R50                    & \multicolumn{1}{c|}{75}       & 43.0 & 64.6      & 45.7     & 22.0   & 46.2    & 61.5    \\ \hline
DETR-DC5-R50                     & \multicolumn{1}{c|}{500}      & 43.3 & 63.1      & 45.9     & 22.5   & 47.3    & 61.1    \\
DETR-DC5-R50                     & \multicolumn{1}{c|}{50}       & 36.7 & 57.6      & 38.2     & 15.4   & 39.8    & 56.3    \\
Conditional DETR-DC5-R50         & \multicolumn{1}{c|}{50}       & 43.8 & 64.4      & 46.7     & 24.0   & 47.6    & 60.7    \\
Conditional DETR-DC5-R50         & \multicolumn{1}{c|}{75}       & 44.5 & 65.2      & 47.3     & 24.4   & 48.1    & 62.1    \\
Conditional DETR-DC5-R50         & \multicolumn{1}{c|}{108}      & 45.1 & 65.4      & 48.5     & 25.3   & 49.0    & 62.2    \\
Pair DETR-DC5-R50                & \multicolumn{1}{c|}{50}       & 44.6 & 65.4      & 47.5     & 24.5   & 48.1    & 61.9    \\
Pair DETR-DC5-R50                & \multicolumn{1}{c|}{75}       & 45.5 & 66.0      & 47.9     & 24.8   & 48.5    & 62.4    \\ \hline
DETR-R101                        & \multicolumn{1}{c|}{500}      & 43.5 & 63.8      & 46.4     & 21.9   & 48.0    & 61.8    \\
DETR-R101                        & \multicolumn{1}{c|}{50}       & 36.9 & 57.8      & 38.6     & 15.5   & 40.6    & 55.6    \\
Conditional DETR-R101            & \multicolumn{1}{c|}{50}       & 42.8 & 63.7      & 46.0     & 21.7   & 46.6    & 60.9    \\
Conditional DETR-R101            & \multicolumn{1}{c|}{75}       & 43.7 & 64.9      & 46.8     & 23.3   & 48.0    & 61.7    \\
Conditional DETR-R101            & \multicolumn{1}{c|}{108}      & 44.5 & 65.6      & 47.5     & 23.6   & 48.4    & 63.6    \\
Pair DETR-R101                   & \multicolumn{1}{c|}{50}       & 43.6 & 64.8      & 46.7     & 22.4   & 47.2    & 62.0    \\
Pair DETR-R101                   & \multicolumn{1}{c|}{75}       & 44.4 & 65.8      & 47.4     & 24.3   & 48.4    & 62.7    \\ \hline
DETR-DC5-R101                    & \multicolumn{1}{c|}{500}      & 44.9 & 64.7      & 47.7     & 23.7   & 49.5    & 62.3    \\
DETR-DC5-R101                    & \multicolumn{1}{c|}{50}       & 38.6 & 59.7      & 40.7     & 17.2   & 42.2    & 57.4    \\
Conditional DETR-DC5-R101        & \multicolumn{1}{c|}{50}       & 45.0 & 65.5      & 48.4     & 26.1   & 48.9    & 62.8    \\
Conditional DETR-DC5-R101        & \multicolumn{1}{c|}{75}       & 45.6 & 66.5      & 48.8     & 25.5   & 49.7    & 63.3    \\
Conditional DETR-DC5-R101        & \multicolumn{1}{c|}{108}      & 45.9 & 66.8      & 49.5     & 27.2   & 50.3    & 63.3    \\
Pair DETR-DC5-R101               & \multicolumn{1}{c|}{50}       & 45.7 & 66.4      & 48.9     & 26.4   & 49.3    & 63.6    \\
Pair DETR-DC5-R101               & \multicolumn{1}{c|}{75}       & 46.1 & 67.2      & 49.3     & 26.7   & 49.8    & 63.9    \\ \hline
Other Single-scale DETR variants &                               &      &           &          &        &         &         \\ \hline
Deformable DETR-R50-SS           & \multicolumn{1}{c|}{50}       & 39.4 & 59.6      & 42.3     & 20.6   & 43.0    & 55.5    \\
UP-DETR-R50                      & \multicolumn{1}{c|}{150}      & 40.5 & 60.8      & 42.6     & 19.0   & 44.4    & 60.0    \\
UP-DETR-R50                      & \multicolumn{1}{c|}{300}      & 42.8 & 63.0      & 45.3     & 20.8   & 47.1    & 61.7    \\ \hline
Deformable DETR-DC5-R50-SS       & \multicolumn{1}{c|}{50}       & 41.5 & 61.8      & 44.9     & 24.1   & 45.3    & 56.0    \\ \hline
\end{tabular}\label{comparetoDETR}
\end{table*}

Two parallel decoders are employed in Pair DETR. Feature maps generated from the encoder are used as common keys by the two decoders. Two decoders are designed to detect top-left and center points, respectively. Each decoder has its own classification and regression loss and both decoders are trained jointly. The same set of learnt positional encodings that are referred to as object queries are fed to the pair of decoders (i.e, top-left decoder and center decoder). Specifically, the first object query from this set which is fed to the top-left decoder will be specialized in detecting the top-left of first bounding box. In addition, this object query is fed to the center decoder to detect the center of corresponding bounding box.  These two embeddings from the two decoders are constructing the positive pair. Contrastive learning is utilized to keep consistent representation from outputs of two decoders. Given 2N queries and a positive pair, similar to~\cite{chen2020simple,radford2021learning}, we treat one pair as positive and the other 2N-1 queries as negative examples. The procedure is depicted in Figures~\ref{fig:method_overall} and ~\ref{fig:contrastive}.



==> Pair DETR-2/sec/4_results.tex <==
%\input{tab/sota}
%\input{tab/ablations}

\section{Results}
%See \Table{sota} and \Table{ablations}.
%\lorem{5}
\subsection{Dataset}
Same as other work in the DETR family, we conduct experiments on COCO 2017 dataset~\cite{lin2014microsoft}. Our models are trained on the train set, and evaluated on the val set.


\begin{table*}[]
\centering
\caption{A comparison of Pair DETR to multi-scale and higher-resolution DETR variants. Pair DETR is a single-scale approach. However our approach when utilizing high resolution backbone such as DC5-R50 and DC5-R101 outperforms the two multi-scale and higher-resolution DETR variants. This is with using only single scale and without using high resolution encoder.}
\begin{tabular}{lc|llllll}
\hline
Model                     & \#epochs & AP   & AP$_{50}$ & AP$_{75}$ & AP$_S$ & AP$_M$ & AP$_L$ \\ \hline
Faster RCNN-FPN-R50~\cite{ren2015faster} & 36       & 40.2 & 61.0    & 43.8    & 24.2   & 43.5   & 52.0   \\
Faster RCNN-FPN-R50 & 108      & 42.0 & 62.1    & 45.5    & 26.6   & 45.5   & 53.4   \\
Deformable DETR-R50       & 50       & 43.8 & 62.6    & 47.7    & 26.4   & 47.1   & 58.0   \\
TSP-FCOS-R50~\cite{sun2021rethinking}              & 36       & 43.1 & 62.3    & 47.0    & 26.6   & 46.8   & 55.9   \\
TSP-RCNN-R50              & 36       & 43.8 & 63.3    & 48.3    & 28.6   & 46.9   & 55.7   \\
TSP-RCNN-R50              & 96       & 45.0 & 64.5    & 49.6    & 29.7   & 47.7   & 58.0   \\ \hline
Pair DETR-DC5-R50         & 50       & 44.6 & 65.4    & 47.5    & 24.5   & 48.1   & 61.9   \\
Pair DETR-DC5-R50         & 108      & 45.8 & 66.2    & 48.8    & 25.7   & 49.0   & 63.0   \\ \hline
Faster RCNN-FPN-R101      & 36       & 42.0 & 62.5    & 45.9    & 25.2   & 45.6   & 54.6   \\
Faster RCNN-FPN-R101      & 108      & 44.0 & 63.9    & 47.8    & 27.2   & 48.1   & 56.0   \\
TSP-FCOS-R101             & 36       & 44.4 & 63.8    & 48.2    & 27.7   & 48.6   & 57.3   \\
TSP-RCNN-R101             & 36       & 44.8 & 63.8    & 49.2    & 29.0   & 47.9   & 57.1   \\
TSP-RCNN-R101             & 96       & 46.5 & 66.0    & 51.2    & 29.9   & 49.7   & 59.2   \\ \hline
Pair DETR-DC5-R101        & 50       & 45.7 & 66.4    & 48.9    & 26.4   & 49.3   & 63.6   \\
Pair DETR-DC5-R101        & 108      & 46.6 & 67.5    & 49.8    & 27.4   & 50.6   & 64.4   \\ \hline
\end{tabular}\label{othercomparison}
\end{table*}

\subsection{Implementation details}
Pair DETR is based on conditional DETR architecture~\cite{meng2021conditional} and consists of the CNN backbone, transformer encoder, two transformer decoders,  prediction feed-forward networks (FFNs) following each decoder layer (the last decoder layer and the 5 internal decoder layers) with parameters shared among the 6 prediction FFNs. Classification network (FFN) is shared between the two decoders (center and top-left decoders) while the regression network is separated. The hyperparameters are the same as DETR and conditional DETR. Conditional spatial embeddings are employed as the spatial queries for conditional multi-head cross-attention and the combination of the spatial query (key) and the content query (key) is done through concatenation other than addition. 
In the first cross-attention layer there are no decoder content embeddings, we make simple changes based on the DETR implementation: concatenate the positional embedding predicted from the object query (the positional embedding) into the original query (key).

The prediction unit for spatial queries is an FFN and consists of learnable linear projection + ReLU + learnable linear projection: $ \mathrm {s =FFN(o_q)}$. The 2D coordinates are normalized by the sigmoid function to use for forming conditional spatial query.
 
We utilized the Hungarian algorithm to find an optimal bipartite matching between predicted and the ground-truth object following DETR~\cite{carion2020end} and then form the loss function for computing and back-propagate the gradients. We follow Deformable DETR~\cite{zhu2020deformable} to formulate the loss: the same loss function with 300 object queries, the same matching cost function, and the same trade-off parameters; The classification loss function is focal loss~\cite{lin2017focal}, and the box regression loss (including L1 and GIoU~\cite{rezatofighi2019generalized} loss) is the same as DETR~\cite{carion2020end}. Each decoder has its own classification and regression loss. Contrastive loss is also utilized between two decoders. 



\begin{figure*}
\begin{tabular}{cccc}
\includegraphics[width=0.23\textwidth]{experiments_visual/conditional_detr/000000001353.jpg} & \includegraphics[width=0.23\textwidth]{experiments_visual/pair_detr/000000001353.jpg} & \includegraphics[width=0.23\textwidth]{experiments_visual/conditional_detr/000000001296.jpg} & \includegraphics[width=0.23\textwidth]{experiments_visual/pair_detr/000000001296.jpg} \\
(a) Conditional DETR & (b) Ours & (c) Conditional DETR & (d) Ours \\
\includegraphics[width=0.23\textwidth]{experiments_visual/conditional_detr/000000000885.jpg} & \includegraphics[width=0.23\textwidth]{experiments_visual/pair_detr/000000000885.jpg} & \includegraphics[width=0.23\textwidth]{experiments_visual/conditional_detr/000000001268.jpg} & \includegraphics[width=0.23\textwidth]{experiments_visual/pair_detr/000000001268.jpg} \\
(e) Conditional DETR & (f) Ours  & (g) Conditional DETR & (h) Ours \\
\end{tabular}
\caption{{Visual comparison on COCO validation set.} Comparing to conditional DETR~\cite{meng2021conditional}, Pair DETR shows superior performance in detecting objects blending in the background (\ref{visualizatoncoco}a vs. b, \ref{visualizatoncoco}g vs. h), locating smaller objects contained within larger objects (\ref{visualizatoncoco}c vs. d), as well as detecting objects around the boundaries of images (\ref{visualizatoncoco}e vs. f, \ref{visualizatoncoco}g vs. h).}
\label{visualizatoncoco}
\end{figure*}

\if 0
\begin{figure*}
\centering
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/conditional_detr/000000001353.jpg}
\caption{Conditional DETR COCO image 1353}
\label{fig:cond_1353}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/pair_detr/000000001353.jpg}
\caption{Pair DETR COCO image 1353}
\label{fig:pair_1353}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/conditional_detr/000000001296.jpg}
\caption{Conditional DETR COCO image 1296}
\label{fig:cond_1296}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/pair_detr/000000001296.jpg}
\caption{Pair DETR COCO image 1296}
\label{fig:pair_1296}
\end{subfigure}

\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/conditional_detr/000000000885.jpg}
\caption{Conditional DETR COCO image 885}
\label{fig:cond_885}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/pair_detr/000000000885.jpg}
\caption{Pair DETR COCO image 885}
\label{fig:pair_885}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/conditional_detr/000000001268.jpg}
\caption{Conditional DETR COCO image 1268}
\label{fig:cond_1268}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{experiments_visual/pair_detr/000000001268.jpg}
\caption{Pair DETR COCO image 1268}
\label{fig:pair_1268}
\end{subfigure}
\caption{{Visual comparison on COCO validation set.} Comparing to conditional DETR~\cite{meng2021conditional}, Pair DETR shows superior performance in detecting objects blending in the background (Figure~\ref{fig:cond_1353} vs. \ref{fig:pair_1353}, Figure~\ref{fig:cond_1268} vs. \ref{fig:pair_1268}), locating smaller objects contained within larger objects (Figure~\ref{fig:cond_1296} vs. \ref{fig:pair_1296}), as well as detecting objects around the boundaries of images (Figure~\ref{fig:cond_885} vs. \ref{fig:pair_885}, Figure~\ref{fig:cond_1268} vs. \ref{fig:pair_1268}).}
\label{visualizatoncoco}
\end{figure*}
\fi 

Training is performed following the DETR training protocol~\cite{carion2020end}. The backbone is the pretrained model on ImageNet from torchvision with batchnorm layers fixed, and the transformer parameters are initialized using the Xavier initialization scheme~\cite{glorot2010understanding}. The weight decay is set to be $10^{-4}$. The AdamW~\cite{loshchilov2018fixing} optimizer is employed.  The learning rates for the backbone and the transformer are initially set to be $10^{-5}$ and $10^{-4}$, respectively. The dropout rate in transformer is 0.1. The learning rate is dropped by a factor of 10 after 40 epochs for 50 training epochs, after 60 epochs for 75 training epochs, and after 80 epochs for 108 training epochs. We use data augmentation following DETR scheme: resizing the input images whose shorter side is between 480 to 800 pixels while the longer side is by at most 1333 pixels; randomly crop the image such that a training image is cropped with probability 0.5 to a random rectangular patch.
We use the standard COCO to evaluate and report the average precision (AP), and the AP scores at 0.50, 0.75 and for the small, medium, and large objects.




\subsection{Comparison to DETR}

We compare the proposed Pair DETR to the original DETR~\cite{carion2020end} and conditional DETR~\cite{meng2021conditional}. We follow~\cite{carion2020end} and report the results over four backbones: ResNet-50~\cite{he2016deep}, ResNet-101, and their %16×-resolution 
high resolution extensions DC5-ResNet-50 and DC5-ResNet-101.


The corresponding DETR models are named as DETR-R50, DETR-R101, DETR-DC5-R50, and DETR-DC5-
R101, respectively. Our models are named as Pair DETR-R50, Pair DETR-R101, Pair DETR-DC5-R50, and Pair DETR-DC5-R101, respectively. 

Table \ref{comparetoDETR} presents the results from DETR, conditional DETR, and Pair DETR. DETR with 50 training epochs performs much worse than 500 training epochs. Conditional DETR with 50 training epochs for R50 and R101 as the backbones performs slightly worse than DETR with 500 training epochs. However Pair DETR (backbone R50 and R101) performs slightly better than DETR with 500 training epochs. In addition, Pair DETR with 50 training epochs for DC5-R50 and DC5-R101 could outperform DETR with 500 training epochs by a bigger margin. Pair DETR for the three backbones with 50 training epochs performs slightly better than conditional DETR with 75 training epochs (the only exception is backbone R101). Figure \ref{visualizatoncoco} visualizes the detection performance of Pair vs. conditional DETR on COCO dataset with 50 training epochs. In addition, Pair DETR with 75 training epochs outperform conditional DETR with 75 training epochs with a larger margin and for all the four backbones. In summary, training Pair DETR for all the backbones is at least 10$\times$ faster than the original DETR. In addition, training Pair DETR for all the backbones is 1.5$\times$ faster than corresponding conditional DETR.
   

\newpage
\begin{table*}[]
\centering
\caption{A comparison of different settings for Pair DETR. We investigate the effect of adding each component to the proposed Pair DETR. Addition of contrastive learning showed effective improvement. In addition, localization of bounding boxes based on two points is more accurate compared to regressing it directly from the center.}
\begin{tabular}{lccc|llllll}
\hline
Model         & Cont. learning & w, h         & Pairs coordinates  & AP   & AP$_{50}$ & AP$_{75}$ & AP$_S$ & AP$_M$ & AP$_L$ \\ \hline
Pair DETR-R50 (a) &                & $\checkmark$ &                        & 41.1 & 62.1    & 43.5    & 20.9   & 44.8   & 59.3   \\
Pair DETR-R50 (b) & $\checkmark$   & $\checkmark$ &                         & 41.8 & 63.3    & 44.1    & 21.1   & 45.2   & 60.7   \\
Pair DETR-R50 (c) & $\checkmark$   &              & $\checkmark$            & 42.1 & 63.6    & 44.5    & 21.3   & 45.4   & 61.0   \\
Pair DETR-R50 (d) & $\checkmark$   & $\checkmark$ & $\checkmark$            & 42.2 & 63.8    & 44.5    & 21.5   & 45.5   & 61.1   \\ \hline
\end{tabular}
\label{Tableablation1}
\end{table*}


\begin{table*}[]
\centering
\caption{A comparison of different matching strategies for Pair DETR.}
\begin{tabular}{lcccc|llllll}
\hline
Model    & head sep.    & head sh.  & Tl cl. cost  & Cent. cl. cost & AP   & AP$_{50}$ & A$_{75}$ & AP$_S$ & AP$_M$ & AP$_L$ \\ \hline
Pair DETR-R50 (1) & $\checkmark$ &              & $\checkmark$ & $\checkmark$   & 41.4 & 62.5      & 43.8     & 21.0   & 44.9   & 59.8   \\
Pair DETR-R50 (2) &              & $\checkmark$ & $\checkmark$ & $\checkmark$   & 42.0 & 63.4      & 44.2     & 21.3   & 45.3   & 60.7   \\
Pair DETR-R50 (3) &              & $\checkmark$ &              & $\checkmark$   & 42.2 & 63.8      & 44.5     & 21.5   & 45.5   & 61.1  
\\ \hline
\end{tabular}
\label{ablation2table}
\end{table*}
In addition, we report the results of single-scale DETR
extensions: UP-DETR~\cite{dai2021up} and deformable DETR-SS~\cite{zhu2020deformable} in Table \ref{comparetoDETR}. Our results over R50 and DC5-R50 are better than deformable DETR-SS: 42.2 vs. 39.4 and 44.6 vs. 41.5. 
%The comparisons might not be fully fair as the Pair DETR is bigger than conditional DETR and DETR and also has different computational complexity compared to deformable DETR, but it implies that having extra decoder to detect corner point is beneficial. 
The comparison might not be fully fair as for example parameter and computation complexities are more different in these extensions, but it implies that the conditional cross-attention mechanism is beneficial. Compared to UP-DETR-R50, our results with fewer training epochs are obviously better.

Overall, some people may take the higher AP in Table~\ref{comparetoDETR} as granted as Pair DETR obviously has more parameters than some of the other methods, e.g., the original DETR and the Conditional DETR, to fit the data. However, in addition to accuracy, it is important to read it from another perspective: Pair DETR demonstrates significantly faster convergence than its counterparts, although having a larger size of model. 


\subsection{Comparison to multi-scale and higher-resolution DETR variants}

It has been shown in prior work that conventional wisdom in computer vision such as embracing higher resolution and multi scale can also boost object detection accuracy for DETRs. %In general we do not expect Pair DETR achieves on par with DETR variants with multi-scale attention and 8×-resolution encoders, e.g., TSP-FCOS and TSP-RCNN~\cite{sun2021rethinking} and deformable DETR~\cite{zhu2020deformable}. %These models were able to reduce the encoder computational complexity and improved the performance due to multi-scale and higher-resolution. 
As they are techniques orthogonal to this paper, it is possible for future extension of Pair DETR also benefits from multi-scale attention and/or higher-resolution encoder. Although we did not perform these implementations, Table \ref{othercomparison} lists the performance of these methods and Pair DETR using higher resolution backbones as a comparison. It can be seen that our methods are on par or better than these recent work. 

%The comparisons in Table \ref{othercomparison} show that our approach on DC5-R50 (16$\times$) outperforms deformable DETR-R50 (multi-scale, 8$\times$). Our model with DC-R50 and DC-R101 and without using multi scaling or high resolution encoder outperforms all the multi-scale models. The only exception is TSP-RCNN which is on par with our model and is trained with almost twice number of epochs (96 epochs). 


%By comparing the Deformable DETR results from Table \ref{comparetoDETR} and \ref{othercomparison} which is 41.5 vs. 43.8,  it is observable that multi-scaling and high resolution encoder is more beneficial for Deformable DETR comparing to high resolution backbone. As diagonal techniques, multi-scale and higher-resolution encoder can also potentially benefit Pair DETR approach. We leave it as future work.
%The performance of our approach is also on par with TSP-FCOS and TSP-RCNN. The two methods contain a transformer encoder over a small number of selected positions/regions (feature of interest in TSP-FCOS and region proposals in TSP-RCNN) without using the transformer decoder, are extensions of FCOS~\cite{tian2019fcos} and Faster RCNN~\cite{ren2015faster}.


\subsection{Ablation}
\textbf{Effect of contrastive loss and regressing bounding box.} We consider four different models to study the effect of different components of the Pair DETR. All models are trained for 50 epochs and the classification head is shared between two decoders. However, each decoder has it own regression head. In the setting (a) contrastive learning is not employed and also (w, h) is used to regress the bounding box from its center. This model performance is very similar to the conditional DETR. 

In second setting (b), the model is jointly trained using contrastive loss and the classification and regression loss functions. Adding contrastive loss function causes the decoders embedding subspace to be more discriminative and consequently the detection performance is improved. In the third setting (c), we utilize the coordinates of two points to measure width and height instead of regressing them directly from the center points. Therefore the conversion function becomes:
\begin{align}\label{coordinates}
	  \mathrm{T(w,h)} = \Big(\mathrm{(x_{tl}-x_{c})} \times 2 , \mathrm{(y_{tl}-y_{c})} \times 2 \Big),
\end{align}
where $(\mathrm{x_{tl}, y_{tl}})$ and $(\mathrm{x_{c}, y_{c}})$ are the coordinates of top-left and center points, respectively. This conversion makes the model to consider two important points instead of relying on one point (center) and it has a positive impact on the detection performance. In the last setting (d), width and height are extracted using Eq.\ref{coordinates} and also predicted independently from center decoder. The conversion function for width and height is taking average of them as follows:
\begin{align}
	  \mathrm{T(w,h)} = \Big(\dfrac{\mathrm{(x_{tl}-x_{c})} \times 2 + \mathrm{w_c}}{2} , \dfrac{\mathrm{(y_{tl}-y_{c})} \times 2 + \mathrm{h_c}}{2} \Big),
\end{align}\label{coordinates_2}
where $(\mathrm{x_{tl}, y_{tl}})$ and $(\mathrm{x_{c}, y_{c}})$ are the coordinates of top-left and center points, respectively. $(\mathrm{w_{c}, h_{c}})$ is the predicted width and height from the center decoder. This setting outperforms the other settings as it is presented in Table \ref{Tableablation1}. 
Here we take the average of the calculated (w,h) from the pair coordinates as well as the predicted width and height from the center decoder. 

\textbf{Strategies for Hungarian matching.}
We evaluate different strategies for Hungarian matching. As it is explained in original DETR paper, after the bounding box prediction step, they are selected in a way to minimize the classification and regression costs. In this experiment, we are interested to explore the effect of classification cost on Hungarian matching and model performance. Three different settings are considered and in all of them the model is trained with 50 training epochs. In the first setting (1), each decoder has its own classification head. Moreover, Top-left decoder has the same role as center decoder in classification cost of Hungarian matching. This model performs worst among all the three settings. In the second setting (2), the classification head is shared between two decoders, but still the classification cost of Top-left decoder plays equal role and is considered in matching. In the third setting (3), the classification head is shared and only the classification cost of center decoder is considered for matching. As it is shown in Table \ref{ablation2table}, this model outperforms the other two settings. One possible reason for this can be due to the fact that the center points contain more representative features related to the content (class id) of the bounding box compared to extreme points or corner points. Therefore this setting is selected for our proposed Pair DETR model. 


==> Pair DETR-2/sec/5_conclusions.tex <==
\section{Conclusions}
%\lorem{3}
In this work, we introduce a simple approach for considering extra point in DETR which detects objects using a pair, including one center keypoint and one corner (Top-left). For this purpose, one additional decoder is employed.
Using this approach, we leverage more than one keypoint for the localization of a bounding box. In addition, we utilize a contrastive learning approach as an auxiliary task to make the output embeddings of two decoders to be more discriminative. Although the presented implementation is based upon conditional DETR, the simplicity of the idea allows it easily extended to other DETR family detectors e.g., Deformable DETR~\cite{zhu2020deformable} in the future, expectably boosting the performance of the base detector by a considerable margin.

==> Pair DETR-2/sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
